Bi-Lipschitz extensions and outlier embeddings into trees

We develop low distortion embeddings with outliers from arbitrary metrics into hierarchically separated trees (HSTs). In particular, we develop an efficient algorithm that for any $\epsilon>0$, given an input metric $(X,d)$, and a probabilistic embedding of all but $k$ points from $X$ into HSTs with distortion $c$, samples from a probabilistic embedding of all but $O(\frac{k}{\epsilon}\log k)$ points into HSTs that achieves distortion at most $(32+\epsilon)c$. Our results are based on two key technical components. First, we extend an algorithm of Munagala et al. [2023] for minimizing the distortion of embeddings without outliers into HSTs to the setting with outliers. We combine this with new results on bi-Lipschitz extensions into trees and $\ell_1$ space. In particular, we show that any probabilistic embedding into HSTs can be extended to $k$ additional points with only a factor $O(\log k)$ of additional distortion. This bi-Lipschitz extension result utilizes a new probabilistic partitioning scheme that we call onion partitioning.

==> alg_bilipl1.tex <==
\begin{algorithm}
\caption{{\bf Bi-Lipschitz extensions for $\ell_1$}}
\label{alg:bilipl1}
\textbf{Input:} Metric space $(X,d)$, subset $S\subseteq X$, embedding $\alpha_S:S\rightarrow \ell_1$


\textbf{Output:} An embedding $\alpha:X\rightarrow \ell_1$

\begin{algorithmic}[1]
\State $T\leftarrow \set{t\in S|\exists X\in K,d(t,x)=d(x,S)}$ \Comment{Use distance tie-breakers so that there is at most one $t$ with $d(t,x)=d(x,S)$}
\State Use terminal set $T$ to find a CKR partition $\set{K_t}_{t\in T}$ of $K=X\setminus S$
\State Create a new embedding $\alpha_S'$ such that $\alpha_S'(u)=\alpha_S(u)$ for all $u\in S$
\State For each $x\in X$, define $\alpha_S'\leftarrow \alpha_S(t)$
\For{$t\in T$}
\State Let $\alpha_t':K_t\rightarrow \ell_1$ be an expanding embedding of $K_t$ into $\ell_1$ with distortion $O(\log |K_t|)$ \Comment{This must exist, by Bourgain \cite{bourgain1985}}
\State Create a new embedding $\alpha_t:K_t\cup\set{t}\rightarrow \ell_1$ 
\State For each $x\in K_t$, set $\alpha_t(x)\leftarrow \alpha_t'(x)|0$ \Comment{Here, $|$ denotes concatenation}
\State Let $t'\in \arg\min_{x\in T}\set{d(x,t)}$
\State For all $x\in X\setminus K_t$, set $\alpha_t(x)\leftarrow \alpha_t'(t')|d(t,t')$
\State Translate the embedding $\alpha_t'$ so that $\alpha_t'(x)$ is at the origin for all $x\in X\setminus K_t$
\EndFor
\State For all $x\in X$, let $\alpha(x)$ be the concatenation of $\alpha_S'(x)$ and $\alpha_t(x)$ for all $t\in T$
\State Return $\alpha$
\end{algorithmic}
\end{algorithm}

==> alg_extend_old.tex <==
\begin{algorithm}
\caption{{\bf Nested Composition:} Algorithm for finding a composition of probabilistic nested embeddings}
\label{alg:nest}
\textbf{Input:} Metric space $(X,d)$, subset $S\subseteq X$, $k=|X\setminus K|$;  Assortment of embeddings $(\cD_S, \set{\cD_{K'}}_{|K'|\leq k+1})$ where $\cD_S: S\rightarrow \cY$ and $\cD_{K'}: K'\rightarrow \cY$ for $K'\subset X$; A function $\pmerge$ that takes in two deterministic embeddings $\alpha:Z\rightarrow \cY$ and $\alpha':Z'\rightarrow \cY$ for $Z, Z'\subset X$ and $|Z\cap Z'|=1$, and returns an embedding $\alpha'':Z\cup Z' \rightarrow \cY$.




\textbf{Output:} A randomly sampled embedding $\alpha:X\rightarrow \cY$.
\begin{algorithmic}[1]
\State $K\from X\setminus S$.
\State \change{Sample $\alpha_S\from \cD_{S}$} 
\State $T\leftarrow \set{s\in S|d(x,s)=d(x,S)}$ \Comment{As before, we assume each $x$ has a unique such $s$ }
\State Let $\set{K_t}_{t\in T}$ be a randomly chosen CKR partition on $(X,S,T)$.
\State Initially, let $\alpha\leftarrow \alpha_S$
\For{$t\in T$}
\State \change{Sample 
        $\alpha_t\from \cD_{K_t}$ }
\State \change{Let $t'\in \arg\min_{x\in K_t}\set{d(x,t)}$} \Comment{This may not be the nearest neighbor of $t$ in $K$, as that node may not be in $K_t$}
\State \change{Let $\alpha'$ be an expanding embedding of $\set{t,t'}$ into a space in $\cY$ with expansion $O(1)$}
\State \change{$\alpha_t\leftarrow \pmerge(\alpha_t,\alpha')$}
\State \change{$\alpha\from \pmerge(\alpha,\alpha_t)$} \label{step:merge}
\EndFor
\State Return $\alpha$
\end{algorithmic}
\end{algorithm}

==> alg_extendhst.tex <==
\begin{algorithm}
\caption{{\bf Bi-Lipschitz extensions for HST embeddings}}
\label{alg:biliphst}
\textbf{Input:} Metric space $(X,d)$, subset $S\subseteq X$, probabilistic embedding $\cD_S:S\rightarrow $ HSTs


\textbf{Output:} An embedding $\alpha:X\rightarrow $ HSTs

\begin{algorithmic}[1]
\State $K\leftarrow X\setminus S$
\State $T\leftarrow \set{t\in S|\exists X\in K,d(t,x)=d(x,S)}$ 
\State Let $\set{K_{t,i}}_{t\in T,i\in [\lceil \log \Delta \rceil]}$ be a random scale partition of $K$, using $T$ as the terminal set; let $\beta$ be as chosen in the partitioning
\State Sample $\alpha_S\leftarrow \cD_S$; let this be our initial embedding $\alpha$
\For{$t\in T,i\in [\lceil \log \Delta \rceil ]$}
\State Sample an embedding $\alpha_{t,i}:K_{t,i}\rightarrow$ HSTs from an FRT embedding
% \State Let $\Delta_{t,i}$ be the diameter of $K_{t,i}$
\State Find the first ancestor, $a$, of $t$ with a label at least $8\cdot \beta \cdot 2^i$
% \State Alter $\alpha$ by making a child of $\alpha$ the root of the tree mapped to by $\alpha_{t,i}$
\State Alter $\alpha$ by ``merging'' $a$ with the root of the tree mapped to by $\alpha_{t,i}$
\State That is, we let the children of $a$ be its own children, plus all children of the root of the tree $\alpha_{t,i}$ maps to
\State Note that $\alpha$ now includes all of $K_{t,i}$ in its domain
\EndFor
\State Return $\alpha$
\end{algorithmic}
\end{algorithm}

==> algnest.tex <==
\begin{algorithm}
\caption{{\bf Nested Composition:} Algorithm for finding a composition of probabilistic nested embeddings}
\label{alg:nest}
\textbf{Input:} Metric space $(X,d)$, subset $S\subseteq X$, $k=|X\setminus K|$;  Assortment of embeddings $(\cD_S, \set{\cD_{K'}}_{|K'|\leq k+1})$ where $\cD_S: S\rightarrow \cY$ and $\cD_{K'}: K'\rightarrow \cY$ for $K'\subset X$; A function $\pmerge$ that takes in two deterministic embeddings $\alpha:Z\rightarrow \cY$ and $\alpha':Z'\rightarrow \cY$ for $Z, Z'\subset X$ and $|Z\cap Z'|=1$, and returns an embedding $\alpha'':Z\cup Z' \rightarrow \cY$.

% \begin{itemize}
%     \item 
%     \item
%     \item 
%     %on sets $Z,Z'$ into $Y$ and $Y'$ respectively, such that $Z\cap Z'=\set{v}$ for some single node $v$; $\merge$ should also take in $v$ (the name of this node) and it should output a new embedding of $Z\cup Z'$ into some $Y''\in \cY$
% \end{itemize}



\textbf{Output:} A randomly sampled embedding $\alpha:X\rightarrow \cY$.
\begin{algorithmic}[1]
\State $K\from X\setminus S$.
\State \change{Sample $\alpha_S\from \cD_{S}$} 
% \Comment{In this algorithm, red text denotes the changes from the algorithms of \cite{chawla2024}}
\State \label{def-gamma-full}Define a function $\neigh:K\fto S$ such that 
$\gamma(u)\in\arg\min_{v\in S} d(u,v)$.
%$\gamma(u)\mapsto v$ where $v$ is an arbitrary vertex in $S$ such that $d(u,S)=d(u,v)$. 
\Comment{i.e. $\neigh(u)$ is one of $u$'s closest neighbors in $S$}
\State Select $\decider$ uniformly at random from the range $[2,4]$
% \State \change{For all $u\in X\setminus S$, create a dummy node $z_u$ and set $d(z_u,v)=d(u,v)$ for all $v\in X$}
\State Select a uniformly random permutation $\perm:K\rightarrow [k]$ of the vertices in $K$
\State $K'\from K,i\from 1,\alpha\from \alpha_S$
\For{$i=1$ to $k$}
    \State\label{ui-def-full} $u_i\from \pi^{-1}(i)$ 
    \State\label{def-ki-full} $K_i\from \{v\in K' \ | \ d(v,u_i)\leq b\cdot d(v,\neigh(v))\}$ \Comment{Let  the ``center" of $K_i$ be $u_i$ } 
    % \State\change{ $K_i\st\leftarrow \begin{cases}
    %     K_i\cup \set{\gamma(u_i)} & i\in K_i \\
    %     K_i\cup \set{\gamma(u_i),z_{u_i}} & u_i\notin K_i,
    % \end{cases}$}

    \State \change{Sample 
        $\alpha_i\from \cD_{K_i\cup\set{\gamma(u_i)}}$  
    }
    
    \State \change{$\alpha\from \pmerge(\alpha,\alpha_i%,\gamma(u_i)
    )$} \label{step:merge}
    \State $K'\from K'\setminus K_i$
\EndFor
\State Output $\alpha$
\end{algorithmic}
\end{algorithm}

==> bilip_embed.tex <==
\section{A framework for bi-Lipschitz extensions}\label{sec:framework}

In Section \ref{sec:bilip-hst}, we showed how to find bi-Lipschitz extensions for HST embeddings. In this section, we present a more general framework for extending embeddings into metric spaces. In particular, our extension method consisted of two main components:
\begin{enumerate}
    \item We refined CKR to create partitions $K_{t,i}$ for each terminal $i$ that have a limited diameter which is bounded by a constant times the maximum distance from this part of the partition to $t$. 

    \item We ``glued'' smaller embeddings on each $K_{t,i}$ to a larger backbone embedding on $S$.
\end{enumerate}

The first part of this argument is not specific to HST embeddings, and in fact the partitioning method we considered in \Cref{sec:partitions} never looked at an embedding at all -- it just used randomness to partition the set $X\setminus S$. 

Thus, the primary challenge in adapting the results of this paper to other settings is in replacing the ``gluing'' step we presented in \Cref{sec:bilip-hst}. To this end, we will present what we call a ``perfect merge function'', which specifies the properties we need for this gluing step to work. We will address the bounds we can obtain for a bi-Lipschitz extension using such a merge function, and we will consider an alternative merge function for HSTs and show that the bi-Lipschitz extensions for $\ell_1$ from \cite{chawla2024} use essentially this same technique paired with a simple merge function for $\ell_1$.




\begin{definition}[Perfect merge]\label{def:merge-expansion}
Let $Z_1,Z_2\subseteq X$ with $Z_1\cap Z_2 = \{v\}$.
Let $\alpha_1:Z_1\rightarrow Y_1$ and $\alpha_2:Z_2\rightarrow Y_2$ be deterministic expanding embeddings, for $Y_1,Y_2\in \cY$. 
%Let $\mergeplain(\alpha,\alpha',v)$ be a function that outputs an embedding $\alpha:Z_1\cup Z_2\rightarrow Y$ for some $Y\in \cY$.
%Then we say that $\mergeplain$ is a {\em \goodmerge\ merge function} for $(X,d)$ if 
We say that a procedure $\mergeplain$  is a \goodmerge\ merge function for embedding $X$ into $\cY$ if given any pair $\alpha_1$ and $\alpha_2$ of embeddings from subsets of $X$ into $\cY$ satisfying the conditions above, it produces a an embedding $\alpha:Z_1\cup Z_2\rightarrow Y$ for some $Y\in \cY$ such that:
% We say that an embedding $\alpha:Z_1\cup Z_2 \rightarrow Y$ for some $Y\in\cY$ is a {\em \goodmerge\ merge} of $\alpha_1$ and $\alpha_2$ if
% \vspace{-.3cm}
\begin{enumerate}
    \item For all $x,y\in Z_1$, $\dista(x, y)=\dista[\alpha_1](x,y)$.
    \item For all $x,y\in Z_2$, $\dista(x, y)=\dista[\alpha_2](x,y)$.
    \item For $x\in Z_1\setminus\set{v}$ and $y\in Z_2\setminus\set{v}$, we have $\dista(x,y)\geq \max\set{\dista[\alpha_1](x,v),\dista[\alpha_2](v,y)}$.
\end{enumerate}
% We say that a procedure $\mergeplain$  is a \goodmerge\ merge function for embedding $X$ into $\cY$ if given any pair $\alpha_1$ and $\alpha_2$ of embeddings from subsets of $X$ into $\cY$ satisfying the conditions above, it produces a \goodmerge\ merge of the pair.
\end{definition}


\kristin{pick back up from here - need to modify this to deal with the diameter-bound instead of just sticking a $\log k$ in front of everything}

Now we present Algorithm \ref{alg:nest} that, given an assortment of probabilistic embeddings on subsets of $X$, produces a new embedding that is drawn from a strongly nested composition of the input embeddings. We highlight in red where Algorithm \ref{alg:nest} differs from Algorithm 5.1 in \cite{chawla2024}. In \cite{chawla2024}, the input $\pmerge$ function was merely concatenation of vectors in the $\ell_1$ metric. We will develop a different \pmerge\ merge function for embeddings into HSTs in this section.



\input{alg_extend_old}


\kristin{now we can adapt the expansion upper bound to this setting, and we can move the contraction bound over from the old version of the paper }


\subsection*{Examples of perfect merge functions}


\kristin{go over why the perfect merge function for $\ell_1$ as just a concatenation of vectors works, and go over the version we presented for HSTs; likely defer proofs to the appendix}



==> bilip_examples.tex <==
\section{Bi-Lipschitz extensions for HSTs}\label{sec:bilip-hst}

With our scale partitioning method in hand, we are now ready to define an algorithm for sampling from a bi-Lipschitz extension of an HST embedding. Algorithm \ref{alg:biliphst} describes this sampling algorithm in detail, but we first discuss a high-level overview of the algorithm.


\begin{enumerate}
% \item \textbf{Partitioning} We begin by using the partitioning method from the previous section to find a partitioning $\set{K_{t,i}}$ of $K=X\setminus S$
\item \textbf{Backbone selection ($\alpha_S$):}
We now select our ``backbone'' embedding by sampling an embedding on the set $S\subseteq X$. This gives us an HST with the nodes of $S$ at the leaves. (Recall that in this paper, we assume that the labels of an HST are powers of $2$, with the leaves having labels $1/2$.)
		
\item \textbf{Scale-Dependent Local mappings ($\alpha_{t,i}$):} 
We use the partitioning method from the previous section to find a partitioning $\set{K_{t,i}}$ of $K=X\setminus S$, where the terminal set is the ``nearest neighbors'' in $S$ of the nodes in $K= X\setminus S$.

Then we use FRT embeddings \cite{frt04} to sample individual embeddings $\alpha_{t,i}$ for each part of the partition with $O(\log |K_{t,i}|)$ expected distortion. Crucially, we will assume that the label at the root of the tree is at most twice the diameter of the cluster $K_{t,i}$. If this is not the case, the overall embedding can be improved by lowering the root label and merging nodes of the same label. 

\item \textbf{{\em Multi-Scale Gluing}:} 
We are left with ``gluing'' together our embeddings $\alpha_{t,i}$ and $\alpha_S$. In particular, we treat $\alpha_S$ as our ``backbone'' tree. That is, we consider the HST mapped to by $\alpha_S$. We will ``hang'' the trees mapped to by each $\alpha_{t,i}$ from this backbone. 

In particular, for each choice of $t,i$, the diameter of $K_{t,i}$ is bounded by $8\cdot \beta\cdot 2^i$. so we can assume that the root of the tree mapped to by $\alpha_{t,i}$ is the smallest power of $2$ that is at least $8\cdot \beta\cdot 2^i$. We merge $T$, the tree mapped to by $\alpha$, and $T_{t,i}$, the tree mapped to by $\alpha_{t,i}$, by finding the ancestor of $t$ in $T$ whose label is the same as the root of $T_{t,i}$ and making all of children of $T_{t,i}$'s root children of that ancestor. 

Intuitively, this will ensure distances between pairs of nodes in $T_{t,i}$ are preserved, as are distances between pairs of nodes in $T$. 
Because the diameter of each $T_{t,i}$ is comparable to the distance between any node in $K_{t,i}$ and $t$, the distance between nodes in $K_{t,i}$ and their ``anchor point'' $t$ will close to their true distance in the underlying metric.

% by making the children of the root of the tree mapped to by
		% The final mapping $\alpha$ is constructed by hanging each scale-specific tree from the backbone tree:
		% \begin{itemize}
		% 	\item For each $R_i(s) \neq \emptyset$, find the first ancestor $a_{s,i}$ of $s$ in the backbone tree whose label is $\ge 8\sigma_i$.
		% 	\item The edge from $a_{s,i}$ to its child along the path leading to $s$ is subdivided. A new node, $s_{\mathrm{new},i}$, is introduced on this edge and assigned the label $8\sigma_i$.
		% 	\item The root of the local tree is attached directly to this new node $s_{\mathrm{new},i}$.
		% \end{itemize}
\end{enumerate}


\input{alg_extendhst}



	
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/gluing-construction.pdf}
    \caption{
        \textbf{Backbone HST Multi-Scale Extension.} 
        \textit{Left:} The original input mapping $\alpha_S$ on the set of terminals $S = \{s_1, s_2, s_3, s_4\}$.
        \textit{Right:} The structural realization of the multi-scale gluing. Local mappings for Steiner points ($\alpha_{s_1,i}, \alpha_{s_2,i}, \alpha_{s_4,i}$) are identified with new nodes $s_{\mathrm{new},i}$ introduced at height $8\sigma_i$. Furthermore, a second local mapping $\alpha_{s_1,j}$ belonging to the same survivor $s_1$ but at a smaller scale $j$ is introduced at a lower height $8\sigma_j$, demonstrating the scale-dependent hierarchy.
    }
		\label{fig:backbone_extension}
\end{figure}

We are now ready to bound the distortion for our extension of the probabilistic embedding $\cD_S$. 

\begin{lemma}[Contraction bound]\label{lem:contraction}
Let $(X,d)$ be a metric, $S\subseteq X$, and $\cD_S$ be a probabilistic embedding of $S$ into HSTs. If all embeddings in the support of $\cD_S$ have contraction at most $c'$, then the embedding $\alpha$ returned by Algorithm \ref{alg:biliphst} has contraction at most $2c'$. 
\end{lemma}

\begin{proof}
Let $x,y\in X$. We will divide into cases to bound the contraction between $x$ and $y$.

\begin{enumerate}
    \item Case 1: $x,y\in S$. In this case, the distance between $x$ and $y$ is the same under $\alpha$ as under the $\alpha_S$ we sampled from $\cD_S$, so the contraction is bounded by $c'$.

    % \item Case 2: $x,y\in K_{t,i}$ for some choice of $t,i$. In this case, the distance between $x$ and $y$ under $\alpha$ is the same as under the embedding $\alpha_{t,i}$ sampled from an FRT distribution, which has contraction at most $1$. Thus, their contraction is at most $1$.

    \item Case 2: $x\in S,y\in K$. 

    Let $y\in K_{t,i}$ for some $t,i$. In this case, $d_\alpha(x,y)\geq \max\set{8\cdot \beta \cdot 2^i,d_{\alpha_S}(y,t)}$. The first bound is because the least common ancestor of $y$ and any node in $S$ is at level at least $8\cdot \beta \cdot 2^i$, and the second is because by our construction any ancestor of $y$ that is also an ancestor of some node in $X\setminus K_{t,i}$ must also be an ancestor of $t$.

 
    Note that $d(x,y)\leq d(x,t)+d(y,t)$, so either $d(x,y)\leq 2d(x,t)$ or $d(x,y)\leq 2d(y,t)$. In the first case, we immediately get contraction at most $2c'$ using the bounds on contraction for $\alpha_S$. In the second case, we get contraction at most $2$, because $d(y,t)\leq 2\cdot A_y\leq 2^{i+2}\cdot \beta$. Thus, $d(x,y)\leq 2^{i+3}\cdot \beta =8\cdot \beta\cdot 2^i$. 


    \item Case 3: $x,y\in K$.

    Let $x\in K_{t,i}$ and $y\in K_{t',i'}$. We break into distinct cases.

    \begin{itemize}
        \item Case a: $t=t'$. 

        If $i=i'$, then then $x$ and $y$ incur no contraction, as their distance under $\alpha$ is the same as under $\alpha_{t,i}$, which incurs no contraction (by properties of FRT). 

        If $i\neq i'$, then their distance is $8\cdot \beta \cdot 2^{\max\set{i,i'}}$. Note that $d(x,y)\leq d(x,t)+d(t,y)\leq 8\cdot \beta\cdot 2^i+8\cdot \beta \cdot 2^{i'}\leq 16\cdot \beta \cdot 2^{\max\set{i,i'}}$, so the contraction between $x$ and $y$ is at most $2$.

        \item Case b: $t\neq t'$.

        In this case, the distance between $x$ and $y$ in the final embedding is at least $8\cdot \beta\cdot 2^{\max\set{i,i'}}$ and at least the distance between $t$ and $t'$ under $\alpha_S$, as a common ancestor of $x$ and $y$ must be an ancestor of both $t$ and $t'$, since any common ancestor of $x$ and a node in $X\setminus K_{t,i}$ must be an ancestor of $t$. 

        We get 

        \begin{align*}
            d(x,y) &\leq d(x,t) + d(t,t') + d(t',y) \\
            &\leq 4\cdot 2^i\cdot \beta +4\cdot 2^{i'}\cdot \beta + d(t,t') \\
            &\leq 8\cdot \beta \cdot 2^{\max\set{i,i'}} +d(t,t'),
        \end{align*}

        where the second to last inequality is by Observation \ref{lem:partition-diam}. Thus, we are either in the case that $d(x,y)\leq 2\cdot 8 \cdot \beta \cdot 2^{\max\set{i,i'}} $ or $d(x,y)\leq 2\cdot d(t,t')$. In the first case, the contraction is at most $1$, and in the second case the contraction is at most $2c'$, using the lower bound on contraction between $t$ and $t'$ under $\alpha_S$.
        
    \end{itemize}
    

    
\end{enumerate}
\end{proof}

\begin{lemma}[Expansion bound]\label{lem:expansion}
Let $S\subseteq X$ and let $\cD_S:S\rightarrow$ HSTs be a probabilistic embedding with contraction at most $c_S'$ and expected expansion at most $c_S$. If $\cD$ is distribution Algorithm \ref{alg:biliphst} samples from with these inputs, then for all $x,y\in X$:
\begin{align*}
    \expec_{\alpha\sim \cD}[d_\alpha(x,y)] &\leq O(c_S\cdot \log k)\cdot d(x,y).
\end{align*}
\end{lemma}

\begin{proof}
We first analyze the most general case where both $x$ and $y$ are Steiner points. Denote $\delta = d(x,y)$, and let $i,j,s,t$ be  such that $x\in K_{s,i}$ and $y\in K_{t,j}$. Recall that $A_x = \min_{s \in S} d(x,s)$ is the distance to the nearest terminal (by how we selected the terminals). Assume w.l.o.g. that $A_x \le A_y$ (and thus $i\le j$). By the triangle inequality, $A_y \le A_x + \delta$.
		
The distance $d_\alpha(x,y)$ is upper bounded by $\max\{8\cdot \beta \cdot 2^i, 8\cdot \beta \cdot 2^j, d_\alpha(s,t)\}$, as the least common ancestor of $x$ and $y$ can be no higher than the highest of the following three nodes: (1) the least common ancestor of $x$ and $s$, (2) the least common ancestor of $y$ and $t$, and (3) the least common ancestor of $s$ and $t$.  

The tree embedding of $K_{i,t}$ is attached to the backbone tree at a level with label at most $2\cdot (8\cdot \beta\cdot 2^i)$, and by  \Cref{lem:partition-diam}, $A_x\geq 2^i\cdot \beta$, so we get
\begin{align}
    d_\alpha(x,y)\leq \max\set{16A_x,16A_y,d_{\alpha_S}(s,t)} \leq 16A_y + d_{\alpha_S}(s,t)\label{eq:distance-cap}
\end{align}


\kristin{I lost a factor of $2$ here, which comes from embedding into exact $2$-HSTs and thus potentially needing to double the diameter, but we could write it for non-exact HSTs if preferred }

We split the analysis into two cases based on the distance $\delta$ relative to the nearest terminals:
		
\textbf{Case 1: Large distance} ($\delta > \frac{1}{4} A_x$).
Since $A_x < 4\delta$, we have $A_y \le A_x + \delta < 5\delta$. By the worst-case proximity of CKR, the metric distance between their assigned terminals is bounded by $d(s, t) \le 2A_x + \delta + 2A_y < 2(4\delta) + \delta + 2(5\delta) = 19\delta$. Taking the expectation over the backbone distribution $\mathcal{D}_S$:
\begin{align*}
    \expec[d_\alpha(x,y)] &\underset{(\ref{eq:distance-cap})}{\le} 16A_y + \expec[d_\alpha(s,t)] \\
    &\le 80\delta + c_S \cdot d(s,t) \\
    &\le 80\delta + c_S \cdot 19\delta \;=\; O(c_S) \cdot d(x,y).
\end{align*}
This directly bounds the expected distance by $O(c_S) \cdot d(x,y)$,  avoiding any $\log k$ penalty in this case.

\textbf{Case 2: Small distance} ($\delta \le \frac{1}{4} A_x$).

Let $\phi(x,y)$ denote the event that $x$ and $y$ are separated by the refined CKR partitioning. By \Cref{lem:scale-separation}, the probability of $\phi(x,y)$ is upper bounded by $O(\log k)\cdot \frac{\delta}{A_x}$. 



% $x$ and $y$ can be separated into different local trees either by the randomized scale partition ($i \neq j$) or subsequently by the CKR rounding ($r(x) \neq r(y)$). Let $\phi(x,y)$ denote the event that $x$ and $y$ are separated by either mechanism.
		
% By \Cref{lem:scale-separation}, the probability they are separated by the scale partition is bounded by $\Pr[i \neq j] \le O\left(\frac{\delta}{A_x}\right)$.

% By \Cref{lem:ckr_separation}, the probability they are separated by the CKR rounding is $\Pr[r(x) \neq r(y)] \le 4\mathcal{H}_m \left( \frac{\delta}{A_x} + \frac{\delta}{A_y} \right) \le O(\log k) \cdot \frac{\delta}{A_x}$. By a union bound, the total probability of separation is $p := \Pr[\phi(x,y)] \le O(\log k) \cdot \frac{\delta}{A_x}$.

% When $\neg\phi(x,y)$ occurs, $x$ and $y$ reside in the exact same local FRT tree, which guarantees an expected distance of at most $O(\log k) \cdot \delta$. 
When $\neg \phi(x,y)$ occurs, $x$ and $y$ are in the same subset $K_{t,i}$, so their expected distance is at most $O(\log k)\cdot \delta$, by the properties of FRT embeddings and the fact that the randomness in the FRT embedding we use is independent of the randomness we used to determine partitions. 
When $\phi(x,y)$ occurs, we rely on our worst-case structural bound. 
Because $\delta \le \frac{1}{4}A_x$, we know $A_y \le A_x + \delta \le \frac{5}{4}A_x = O(A_x)$. Similarly, $d(r(x),r(y)) \le 2A_x + \delta + 2A_y \le \frac{19}{4}A_x = O(A_x)$. \ytodo{I think r(x) is from previous notation. Maybe need to specify $x\in K_{s,i}~,~y\in K_{t,j}$}
		
We can now cleanly bound the overall expectation:
\begin{align*}
    \mathbb{E}[d_\alpha(x,y)] &= \Pr[\neg\phi] \cdot \mathbb{E}[d_\alpha(x,y) \mid \neg\phi] + \Pr[\phi] \cdot \mathbb{E}[d_\alpha(x,y) \mid \phi] \\
    &\le 1 \cdot \big(O(\log k) \cdot \delta\big) + \Pr[\phi] \cdot \Big( 8A_y + c_S \cdot d(r(x),r(y)) \Big) \\
    &\le O(\log k) \cdot \delta + \left( O(\log k) \cdot \frac{\delta}{A_x} \right) \cdot \Big( O(A_x) + c_S \cdot O(A_x) \Big) \\
    &\le O(\log k) \cdot \delta + O(c_S \cdot \log k) \cdot \delta \\
    &= O(c_S \cdot \log k) \cdot d(x,y).
\end{align*}

The cases where at least one point is a terminal follow directly from this analysis. If $x\in S,y\in K$, this can be analyzed identically to adding a point in $K$ at distance $0$ from $x$. Because $A_x = 0$, the condition $\delta > \frac{1}{4}A_x$ is trivially satisfied, placing us inherently in the "Large distance" regime where everything holds under the worst-case bound without a $\log k$ penalty. Finally, if both $x, y \in S$, they reside entirely in the backbone, meaning their expected distance is strictly bounded by $c_S \cdot d(x,y) \le O(c_S \cdot \log k) \cdot d(x,y)$.    
\end{proof}


Now we are ready to prove that Algorithm \ref{alg:biliphst} samples from the bi-Lipschitz extension outlined in Theorem \ref{thm:bilip-hst}. 

\begin{proofof}{Theorem \ref{thm:bilip-hst}}
Lemmas \ref{lem:contraction} and \ref{lem:expansion} give us the desired contraction and expansion bounds on the embedding sampled by Algorithm \ref{alg:biliphst}, so we are left with  showing that the distribution of distances between points in $S$ is the same under the extension as under the original embedding.

Let $\cD_S$ be the original embedding on $S$, and let $\cD$ be the embedding of $X$ implied by Algorithm \ref{alg:biliphst} with $\cD_S$ as input. Note that if $\alpha_S:S\rightarrow$ HSTs and $\alpha$ is the extension of $\alpha_S$ produced by Algorithm \ref{alg:biliphst}, then the tuples $(d_\alpha(x,y))_{(x,y)\in S\times S}$ and $(d_{\alpha_S}(x,y))_{(x,y)\in S\times S}$ are identical, no matter the randomness of the algorithm, as the distance between points in the backbone never changes when turning $\alpha_S$ into $\alpha$. As Algorithm \ref{alg:biliphst} samples $\alpha_S$ from  $\cD_S$ and extends it, the distribution of $(d_\alpha(x,y))_{(x,y)\in S\times S}$ is the same whether we draw $\alpha$ from $\cD_S$ or from the extension of $\cD$.
\end{proofof}

\begin{remark}
    Full domination (i.e. contraction at most $1$) cannot be achieved under our construction. In our setting, $d_\alpha(x,y)$ is only guaranteed to be at least the \emph{maximum} among its component distances---namely if $x\in K_{s,i},y\in K_{t,j}$, then $d_\alpha(x,s)$, $d_\alpha(s,t)$, and $d_\alpha(t,y)$---but not necessarily their \emph{sum}. For the underlying metric $d$, we only know that it satisfies the triangle inequality, which provides an upper bound by the sum of these components. Consequently, unless we attach the subtree at height exactly $d_\alpha{}(s,t)$, there will always be an additive term (proportional to $2^i$ or $2^j$) contributing to an approximation factor.
\end{remark}

In Appendix \ref{sec:framework}, we further discuss some of the main ideas and how they may adapt to a more general framework for bi-Lipschitz extensions.



==> bilip_examples_old.tex <==
\section{Bi-Lipschitz extensions for HSTs}

\kristin{my initial thinking for $\ell_1$ was not correct - you still get $\log^2k$ if you follow that reasoning}

In this section, we prove the existence of bi-Lipschitz extensions with bounded contraction for $\ell_1$ and show how to sample from such an extension for HSTs. 

\subsection{Extensions for $\ell_1$}

As a warm-up, we begin with $\ell_1$ embeddings. In particular, suppose we have a subset $S\subseteq X$ with an expanding embedding $\alpha_S:S\rightarrow \ell_1$ of distortion at most $c$. Letting $K:=X\setminus S$, we can construct a bi-Lipschitz extension for $\ell_1$. Algorithm \ref{alg:bilipl1} samples from a probabilistic bi-Lipschitz extension for a deterministic embedding $\alpha_S:S\rightarrow \ell_1$. However, due to the following claim from Chawla and Sheridan \cite{chawla2024}, we can conclude that there exists a deterministic bi-Lipschitz extension of $\alpha_S$ with the same extension factors. 


\begin{claim}[Probabilistic embeddings imply deterministic embeddings for $\ell_1$, implicit in \cite{chawla2024}]
Let $\cD:X\rightarrow \ell_1$ be an expanding probabilistic embedding with expected expansion $c$ such that $\cD$ has finite support. Then there exists an expanding deterministic embedding $\alpha:X\rightarrow \ell_1$.

Further, this embedding has the property that for every $x\in X$ with a fixed value of $\alpha'(x)$ for every $\alpha'$ in the support of $\cD$, $\alpha(x)=\alpha'(x)$.
\end{claim}


Algorithm \ref{alg:bilipl1} takes in a metric $(X,d)$, as well as a subset $S\subseteq X$ and an embedding of $S$ into $\ell_1$. It then finds a set of terminals $T$ that are the ``nearest neighbors'' in $S$ of nodes in $K:=X\setminus S$. It finds a CKR partition $\set{K_t}_{t\in T}$ of $K$ using this terminal set and proceeds to find an $O(\log |K_t|)$-distortion $\ell_1$ embedding on each piece of the partition, which must exist (and in fact can be found efficiently with high probability) by Bourgain \cite{bourgain1985}. It ``appends'' the rest of the metric, $X\setminus K_t$ to this embedding on $K_t$ by adding one new index such that each node in $K_t$ has a $0$ on the remaining index, and each node not in $K_t$ has a value $d(t,t')$, where $t'$ is a nearest neighbor of $t$ in the set $K_t$. (Note that the nearest neighbor of $t$ in $K$ is not required to be in $K_t$, so this choice depends on the randomness of the CKR partition.) Further, on the preceding indices, we map each $x\in X\setminus K_t$  to the same  values as $t'$. 

The idea of this method is that in the final embedding $\alpha_t:X\rightarrow \ell_1$, all pairs of nodes in $K_t$ have a distance that is non-contracting and of distortion at most $O(\log |K_t|)$, while all nodes not in $K_t$ are mapped to a spot $d(t,t')$ away from $t'$, and the shortest path from any node in the 




\input{alg_bilipl1}

% \begin{enumerate}
%     \item Let $T\subseteq S$ be the set of ``nearest neighbors'' of nodes in $K$. That is, \\ $T:=\set{t\in S|\exists x\in K,d(t,x)=d(x,S)}$. (We assume we use distance tie-breakers such that for each $x$, only one choice of $t\in S$ has $d(t,x)=d(x,S)$.
    
%     \item Find a CKR partition $\set{K_t}_{t\in T}$ of $K$, with terminal set $T$

%     \item For each $x\in K$, let $\alpha_S'(x):=\alpha_S(t)$, where $x\in K_t$, and let $\alpha_S'(x):=\alpha_S(x)$ for all $x\in S$.

%     \item For each $t\in T$, let $\alpha_t:X\rightarrow \ell_1$ be as follows:
%     \begin{itemize}
%         \item Let $\alpha_t':K_t\rightarrow \ell_1$ be an expanding embedding of $K_t$ into $\ell_1$ with distortion $O(\log |K_t|)$. (Such an embedding must exist by Bourgain \cite{bourgain1985}.)

%         \item For each $x\in K_t$, let $\alpha_t(x):=\alpha_t'(x)|0$, where $|$ denotes concatenation. 
%         \item Let $t'\in \arg\min{x\in K_t}\set{d(t,x)}$, and for all $x\in X\setminus S$ let  $\alpha_t(x):=\alpha_t'(t')|d(t,t')$
%     \end{itemize}
%     \item For all $x\in X$, let $\alpha(x)$ be the concatenation of $\alpha_t(x)$ for all $t\in T$, as well as $\alpha_S'(x)$.
% \end{enumerate}


\kristin{from here, the analysis follows \cite{chawla2024}, except that we take more care in the bad case where we route the path between $x$ and $y$ through their assigned nodes $t_x$ and $t_y$, noting that the distortion between $x$ and $t_x$ in this embedding is $O(1)$ (this will probably need to be a separate lemma) }


\subsection{Extensions for HSTs}

In this section, we prove Theorem \ref{thm:bilip-hst}. In particular, we find CKR partitions of our set $K=X\setminus S$, but we further divide these partitions, using a randomized version of bucketing based on the distance between a node and the set $S$. This additional partitioning increases the probability of a pair $x,y$ being separated under the final partition by only a constant factor, so we will be able to use many of the same bounding techniques of \cite{calinescu2005extension}. We will then ``stitch'' an embedding of each new partition to the original ``good'' HST embedding on $S$. Using the fact that all pairs of nodes in a partition have a similar distance to the set $S$, we can bound the distance that must be traveled between $x$ and $y$ when $x$ and $y$ are separated by bounding (1) the distance $x$ travels back to the backbone embedding, (2) the distance between $x$ and $y$'s assigned terminals in the backbone, and (3) the distance $y$ must travel to the backbone embedding. Notably, none of these distances depend on the $O(\log k)$ distortion factor implied by FRT embeddings, so in our ``bad case'' (where a close pair $x,y$ is separated by the partitioning), we do not need to incur a cost of $O(\log k)$ for the FRT embedding {\em and} an $O(\log k)$ factor from the CKR partition. In fact, we will be able to divide into cases such that the distance between $x$ and $y$ depends only on one of the two $O(\log k)$ factors.



\kristin{import the additional partitioning idea plus backbone stitching concept from the other paper }



==> expansion.tex <==
Notably, this proof follows the same lines as the proof of Lemma 5.2 in \cite{chawla2024}. We only repeat it here for completeness and to clarify or simplify a few places in the lemma proof where terms were stated in a way that specific to $\ell_1$ embeddings or deterministic embeddings. A modification of the expansion proof in Section 2 of Calinescu et al. \cite{calinescu2005extension} could similarly help bound expansion for this algorithm.
We will begin by giving a new version of Lemma 5.2 from \cite{chawla2024}. Note that parts \ref{lem:not-outlier}, \ref{lem:ui}, \ref{lem:farxy}, and \ref{lem:closexy}  together imply Lemma \ref{lem:merge-expansion}. 

\begin{lemma}\label{lem:expansion}
Let $\alpha\from$ Algorithm \ref{alg:nest}$((X,d),\cD_S,\set{D_{K'}},\pmerge)$ where $\pmerge$ is a \goodmerge\ merge function. Let $c_S$ be the distortion of $\cD_S$ and let $c_X(k)$ be an upper bound on the distortion of any embedding in $\set{\cD_{K'}}$. Let $\cD\st$ be the embedding distribution that results from the application of Algorithm \ref{alg:nest}. Then we have the following bounds on the expansion for each pair $x,y\in X$:
\begin{enumerate}[(a)]
    \item \label{lem:not-outlier} If $x,y\in S$, then $$\expec_{\alpha\sim \cD\st}[\dista(x,y)]\leq c_S\cdot d(x,y).$$
    
    \item \label{lem:sameset} If $x,y\in K_i$ for some $K_i$ at step \ref{def-ki-full} of the algorithm, then let $\set{K_j}$ be the full partition of $X\setminus S$ by the algorithm, and we get $$\expec_{\alpha\sim \cD\st}[\dista(x,y)|\set{K_j}]\leq c_X(k)\cdot d(x,y).$$


    
    \item \label{lem:ui} If $y\in X\setminus S$ and $x\in S$, then 
     $$
    \expec_{\alpha\sim \cD\st}[\dista(x,y)] \leq (10c_S+9c_X(k))\cdot d(x,y).
    $$

   

    \item \label{lem:farxy} If $x,y\in X\setminus S$
    { and $d(x,\gamma(x))\leq 2\cdot d(x,y)$ for $\gamma$ as defined in line 2 of the algorithm}, then $$\expec_{\alpha\sim \cD\st}[\dista(x,y)]\leq [50\cdot c_S+45\cdot c_X(k)]\leq d(x,y).$$

    
    \item \label{lem:closexy} If $x,y\in X\setminus S$ { and $d(x,\neigh(x)),d(y,\neigh(y))> 2\cdot d(x,y)$ for $\neigh$ as defined in line 2 of the algorithm}, then 
   
    $$\expec_{\alpha\sim \cD\st}[\dista(x,y)] \leq (125c_S+116c_X(k))\cdot H_k \cdot  d(x,y)$$
\end{enumerate}
\end{lemma}

The proof of each part of this lemma will largely follow that of \cite{chawla2024}, with small changes to account for the input probability distributions of subsets of metrics rather than a single embedding on the entire metric (as well as randomness in the embedding on the good subset), and to account for the fact that we are dealing with a general merge algorithm and host metric, rather than specifically concatenation and $\ell_1$. We have also simplified the proof in a few places.


\begin{proofof}{Lemma \ref{lem:expansion}\ref{lem:not-outlier}}
Note that our initial setting of $\alpha$ is exactly $\alpha_S$. Thus, the distance that $x$ and $y$ incur under $\alpha_S$ is exactly that incurred under the final $\alpha$. Thus by Fact \ref{lem:induct}
\begin{align*}
    \expec_{\alpha\sim \cD\st}[\dista(x,y)] = \expec_{\alpha_S\sim \cD_S}[\dista[\alpha_S](x,y)] \leq c_S\cdot d(x,y),
\end{align*}
where the last line is by definition of $c_S$.
\end{proofof}

\begin{proofof}{Lemma \ref{lem:expansion}\ref{lem:sameset}}
We have $x,y\in K_i$, so $x$ and $y$ are first added to the domain of $\alpha$ in the $i$th iteration of Step \ref{step:merge} in the algorithm. At this point, we set $\alpha \from \pmerge(\alpha,\alpha_i)$, where $x$ and $y$ are in the domain of $\alpha_i$ and $\alpha_i$ is sampled from $\cD_{K_i}$. Due to Fact \ref{lem:induct}, the distance between $x$ and $y$ under $\alpha$ is unchanged after all future steps, and due to the fact we have a $\pmerge$ function, their distance under $\alpha$ at this step is exactly their distance under $\alpha_i$. Thus, by Fact \ref{lem:induct} at this step we get 
\begin{align*}
    \expec_{\alpha\sim \cD\st}[\dista(x,y)|\set{K_j}] = \expec_{\alpha_i\sim \cD_{K_i}}[\dista[\alpha_i](x,y)] \leq c_X(k)\cdot d(x,y),
\end{align*}
where we use the bound on distortion of $\cD_{K_i}$.
\end{proofof}




\begin{proofof}{Lemma \ref{lem:expansion}\ref{lem:ui}}
We begin by bounding $ \expec_{\alpha\sim \cD\st}[\dista(x,y)|\set{K_j}]$, the expectation conditioned on the partition of $\set{K_j}$ of $X\setminus S$. Let $y\in K_i$ for $K_i\in \set{K_j}$. We first focus on bounding the expected distortion between $y$ and $\gamma(u_i)$ (the nearest neighbor of $y$'s cluster's center). 
\begin{align*}
    \expec_{\alpha\sim \cD\st}[\dista(\gamma(u_i),y)|\set{K_j}]] &= \expec_{\alpha_i\sim \cD_{K_i}}[\dista[\alpha_i](\gamma(u_i),y)] \\
    &\leq c_X(k)\cdot d(\gamma(u_i),y),  
\end{align*}

where the first line is by the fact that when $y$ first joins the domain of $\alpha$, it is as a result of $\pmerge(\alpha,\alpha_i)$ for some $\alpha$ where $\gamma(u_i)$ is in the domain of both $\alpha$ and $\alpha_i$. Since \pmerge\ is a \goodmerge\ merge function, we get that the distance between $\gamma(u_i)$ and $y$ is the same as  before the merge. The second line is by the expected distortion of $\cD_{K_i}$.

Now consider a more general $x\in S$. We get 
\begin{align*}
    \expec_{\alpha\sim \cD}[\dista(x,y)|\set{K_j}] &\leq \expec_{\alpha\sim \cD}[\dista(\gamma(u_i),x)|\set{K_j}] + \expec_{\alpha\sim \cD}[\dista(\gamma(u_i),y)|\set{K_j}] \\
    &\leq c_S\cdot d(\gamma(u_i),x) + c_X(k)\cdot d(\gamma(u_i),y) \\
    &\leq c_S\cdot d(x,y) + (c_S+c_X(k))\cdot d(\gamma(u_i),y) \text{ (triangle inequality)} \\
    &\leq c_S\cdot d(x,y) + (c_S+c_X(k))\cdot (d(u_i,\gamma(u_i))+d(u_i,y)) \text{ (triangle inequality)} \\
    &\leq c_S\cdot d(x,y) + (c_S+c_X(k))\cdot (d(u_i,x)+4d(x,y))  \\
    &\leq (5c_S+4c_X(k))\cdot d(x,y) + (c_S+c_X(k))\cdot (d(u_i,y)+ d(x,y)) \text{ (triangle inequality)} \\
    &\leq (6c_S+5c_X(k))\cdot d(x,y) + (c_S+c_X(k))\cdot 4d(x,y)  \\
    &=(10c_S+9c_X(k))\cdot d(x,y).
\end{align*}

The first line here is by the triangle inequality on $\alpha$. The second line is by Lemma \ref{lem:expansion}\ref{lem:not-outlier} and the previous case of this lemma. Lines three, four, and six are by the triangle inequality on $(X,d)$, and the last line is by rearranging. Line five is by the fact that $d(u_i,\gamma(u_i))\leq d(u_i,x)$, as $\gamma(u_i)$ is a closest node in $S$
 to $u_i$ and $x\in S$. The fifth and seventh lines also use the fact that $d(u_i,y)\leq 4d(y,\gamma(y))\leq 4d(y,x)$, as well as the definition of $\gamma(x)$ and the upper bound on $b$ in the algorithm.

Now we show that this inequality still holds when we do not condition on $\set{K_j}$, and we note that the law of total expectation immediately gives us the result. 

\begin{align*}
    \expec_{\alpha\sim \cD\st}[\dista(x,y)] &= \expec_{\set{K_j}}[\expec_{\alpha\sim \cD\st}[\dista(x,y)|\set{K_j}]] \\
    &\leq \expec_{\set{K_j}}[(10c_S+9c_X(k))\cdot d(x,y)] \\
    &= (10c_S+9c_X(k))\cdot d(x,y).
\end{align*}
\end{proofof}




\begin{proofof}{of Lemma \ref{lem:expansion}\ref{lem:farxy}}
We have 
\begin{align*}
    \expec_{\alpha\sim \cD\st}[\dista(x,y)] &\leq \expec_{\alpha\sim \cD\st}[\dista(x,\gamma(x))] + \expec_{\alpha\sim \cD\st}[\dista(y,\gamma(x))] \\
    &\leq (10c_S+9c_X(k))\cdot d(x,\gamma(x)) + (10c_S+9c_X(k))\cdot d(y,\gamma(x)) \\
    &\leq (20c_S+18c_X(k))\cdot d(x,\gamma(x)) + (10c_S+9c_X(k))\cdot d(x,y) \\
    &\leq (50c_S+45c_X(k))\cdot d(x,y), 
\end{align*}
where the first line is by the triangle inequality on $Y(\alpha)$ and linearity of expectation, the second is by Lemma \ref{lem:expansion}\ref{lem:ui}, the third is by the triangle inequality on $(X,d)$, and the fifth is by the condition of this lemma that $d(x,\gamma(x))\leq 2d(x,y)$.
\end{proofof}

Before we prove the last part of the Lemma, we will discuss some of the terminology and results from the proof of Lemma 4.1(d) from \cite{chawla2024}. This will help abbreviate our proof of Lemma \ref{lem:expansion}\ref{lem:farxy} in this paper. 


First, we say that $x,y\in X\setminus S$ are ``split'' if $x\in K_i,y\in K_j$ for $i\neq j$ from Line \ref{def-ki-full} of Algorithm \ref{alg:nest}. Further, we say ``$u$ splits $x$ and $y$'' if $u$ is the first node under the ordering $\pi$ such that exactly one of $x$ and $y$ is in $K_{\pi(u)}$. For a given pair $x,y\in X\setminus S$, we define $\beta_{u,\set{x,y}}:=\min\set{\frac{d(x,u)}{d(x,\gamma(x))},\frac{d(y,u)}{d(y,\gamma(y))}}$. Consider a fixed ordering of the $u\in X\setminus S$ by increasing $\beta_{u,\set{x,y}}$. Then denote the index of $u$ in this ordering as $\ind_{\set{x,y}}(u)$. From \cite{chawla2024} and the fact that partitions in this algorithm are picked the same way as in that paper's Algorithm 4.1, we get the following claim.

\begin{clm}[from \cite{chawla2024}]\label{claim:prob-sep}
For a pair $x,y\in X\setminus K$ and a node $u\in X\setminus K$, let $x_u$ be $\arg\min_{x,y}\set{d(x,u),d(x,y)}$. Then in Algorithm \ref{alg:nest}, we have  $\Pr[x \text{ and }y \text{ are split by }u]\leq 5\frac{d(x,y)}{d(x_u,\gamma(x_u))}\cdot \frac{1}{\ind_{\set{x,y}}(u)}$.
\end{clm}


\begin{proofof}{Lemma \ref{lem:expansion}\ref{lem:closexy}}
Finally, we are left with pairs $x,y\in X\setminus S$ with $d(x,y)\leq d(x,\gamma(x))/2,d(y,\gamma(y))/2$. 
% Note that when $x$ and $y$ are not split, their distance under the final embedding is $0$ (as they are mapped to the same place). 
Consider a set of $\set{K_j}$ that does split $x$ and $y$. We get 

\begin{align*}
    \expec_{\alpha\sim \cD\st}[\dista(x,y)|\set{K_j}] &\leq \expec_{\alpha\sim \cD\st}[\dista(x,\gamma(x))|\set{K_j}] + \expec_{\alpha\sim \cD\st}[\dista(\gamma(x),y)|\set{K_j}] \\
    &\leq (10c_S+9c_X(k))\cdot d(x,\gamma(x)) + (10c_S+9c_X(k))\cdot d(y,\gamma(x)) \\
    &\leq (20c_S+18c_X(k))\cdot d(x,\gamma(x)) + (10c_S+9c_X(k))\cdot d(x,y) \\
    &\leq (25c_S+23c_X(k))\cdot d(x,\gamma(x)),
\end{align*}

where the first line is by linearity of expectation and the triangle inequality on $Y(\alpha)$, the second line is by Lemma \ref{lem:expansion}\ref{lem:ui}, the third is by the triangle inequality on $(X,d)$, and the fourth is by the condition of this lemma that $d(x,y)\leq d(x,\gamma(x))/2$ (and rounding up when dividing odd numbers by $2$). Note that by symmetry, we also get $ \expec_{\alpha\sim \cD\st}[\dista(x,y)|\set{K_j}]\leq (25c_S+23c_X(k))\cdot d(y,\gamma(y))$.

These inequalities hold for {\em every } choice of $\set{K_j}$ that separates $x$ and $y$. Let's consider the expected distance overall for $x$ and $y$, and let $H_k$ be the $k$th harmonic number. We get 
\begin{align*}
 \expec_{\alpha\sim \cD\st}[\dista(x,y)] &= \Pr[x,y\text{ are not split}]\cdot \expec_{\alpha\sim \cD\st}[d_\alpha(x,y)|x,y\text{ are not split}] \\
 &\ \ \ \ \ + \sum_{\set{K_j}\text{ that splits }x,y}\Pr[\set{K_j}]\cdot  \expec_{\alpha\sim \cD\st}[\dista(x,y)|\set{K_j}] \\
 &\leq c_X(k)d(x,y) \\
 & \ \ \ \ \ + \sum_{\set{K_j}\text{ that splits }x,y}\Pr[\set{K_j}]\cdot (25c_S+23c_X(k))\cdot \min\set{d(x,\gamma(x)),d(y,\gamma(y))} \\
 &= c_X(k)d(x,y) +  (25c_S+23c_X(k))\cdot \min\set{d(x,\gamma(x)),d(y,\gamma(y))}\sum_{u\in X\setminus S}\Pr[u\text{ splits }x,y] \\
 &\leq c_X(k)d(x,y) \\
 & \ \ \ \ \ +  (25c_S+23c_X(k))\cdot \min\set{d(x,\gamma(x)),d(y,\gamma(y))}\cdot \sum_{u\in X\setminus S} 5\frac{d(x,y)}{d(x_u,\gamma(x_u))}\cdot \frac{1}{\ind_{\set{x,y}}(u)}\\
 &\leq c_X(k)d(x,y) +  5(25c_S+23c_X(k))\cdot d(x,y)\cdot \sum_{u\in X\setminus S}\frac{1}{\ind_{\set{x,y}}(u)} \\
 &\leq H_k\cdot (125c_S+
116c_X(k))\cdot d(x,y),
\end{align*}

where the first line is by the law of total probability and the fact that the expected distance between $x$ and $y$ is at most $c_X(k)\cdot d(x,y)$ when they are not split, as in all such cases we simply draw an embedding involving $x$ and $y$ from some $\cD_{K}$; 
the second line is by our earlier bound on $\expec_{\alpha\sim \cD\st}[d_{Y(\alpha)}(\alpha(x),\alpha(y))|\set{K_j}]$ and Lemma \ref{lem:expansion}\ref{lem:sameset}; 
the third is by the fact that $(25c_S+23c_X(k))\cdot \min\set{d(x,\gamma(x)),d(y,\gamma(y))}$ has no dependence on $\set{K_j}$ and the fact that $\sum_{\set{K_j}
\text{ that splits }x,y}[\set{K_j}]$ and $\sum_{u\in X\setminus S}\Pr[u\text{ splits }x,y] $ both give the total probability that $x$ and $y$ are split by the algorithm; 
the fourth line is by Claim \ref{claim:prob-sep};
 the fifth line is by the fact that $\frac{\min\set{d(x,\gamma(x)),d(y,\gamma(y))}}{d(x_u,\gamma(x_u))}\leq 1$, as $d(x_u,\gamma(x_u))\in \set{d(x,\gamma(x)),d(y,\gamma(y))}$; and the final line comes from the fact that $\ind_{\set{x,y}}(u)$ ranges over an ordering of the $k$ things in $X\setminus S$.
\end{proofof}


==> lipschitz.tex <==
\section{Probabilistic Lipschitz extensions\label{sec:lip}}

While the primary focus of this paper is on strong nested embeddings and their applications to finding outlier HST embeddings, in this section we will also briefly mention how an ``oblivious'' Lipschitz extension algorithm for deterministic embeddings can also serve as a Lipschitz extension algorithm for probabilistic embeddings. In particular, we consider the case that we have some ``oblivious'' algorithm that takes in a deterministic embedding $\alpha:S\xhookrightarrow{c_S}Y$ for $S\subseteq X$ and samples from a probabilistic Lipschitz extension of that embedding. We will show here that if we have a probabilistic embedding $\cD_S:S\probembed{c_S}\cY$ instead, we can sample any embedding from $\cD_S$ and run the existing Lipschitz extension algorithm on it in order to obtain a sample from a Lipschitz extension of $\cD_S$. Notably, the original Lipschitz extension (and corresponding algorithm) {\em must} be oblivious, in that for each $x\notin S$, the extension always maps $x$ to the same spot as some $u\in S$, and the choice of such $u$ is completely independent of the input embedding $\alpha_S$.  

We first define probabilistic and oblivious Lipschitz extensions. 

\begin{definition}\label{def:oblivious}
A probabilistic Lipschitz extension of a deterministic embedding with extension factor $L$ of a deterministic embedding $\alpha_S:S\xhookrightarrow{c_S}Y$ for some space $Y$ and $S\subseteq X$ is a probabilistic embedding $\cD:X\probembed{} Y$ such that for all $\alpha$ in the support of $\cD$ and all $u\in S$, $\alpha(u)=\alpha_S(u)$; and for all $x,y\in X$ $\expec_{\alpha\sim \cD}[\dista(x,y)]\leq L\cdot c_S\cdot d(x,y)$.
% \footnote{Standard Lipschitz extension definitions deal only with deterministic extensions $\alpha:X\embed{}Y$ and refer to the embedding itself as an extension. We modify this by defining a probabilistic variant and referring to a function $f$ mapping the input embedding $\alpha_S$ to the full embedding $\cD$ as the Lipschitz extension, rather than $\cD$ itself. }


Further, we say that a function $f$ mapping input embeddings $\alpha_S$ to Lipschitz extensions $\cD$ is an{\em oblivious Lipschitz extension function} if for all $x\in X\setminus S$, $\alpha(x)\in \set{\alpha(u):u\in S}$ with probability $1$, and for all $u\in S$, $\Pr_{\alpha\sim f(\alpha_S)}[\alpha(x)=\alpha(u)]$ is the same for all inputs $\alpha_S$.
\end{definition}

Notably, Lipschitz extensions $\alpha$ on deterministic embeddings $\alpha_S$ require that $\alpha(u)=\alpha_S(u)$ for all $u\in S$ with probability $1$. In the randomized setting, $u$ is not mapped to a fixed place in a metric space, so we need to clarify what we mean by a Lipschitz extension. In particular, we will require not only that the distribution of $u$ under the new embedding be the same as under the old embedding, but also that the {\em joint distribution} of the embedding on all points in $S$ is unchanged by the new embedding. Because of this, we get that the output embedding has the same expected distortion on any pair of nodes as under the original embedding, but in fact this is a much stricter requirement.

We define Lipschitz extensions of probabilistic embeddings below.


\begin{definition}
Let $(X,d_X)$ be a metric space, let $\cY$ be a set of metric spaces, and $\cD_S:S\probembed{c_S}\cY$ for $S\subseteq X$. Then $\cD:X\probembed{}\cY$ is a {\em Lipschitz extension} of  $\cD_S$  with extension factor $L$ if:
\begin{enumerate}
\item The distribution of $(\alpha(x_i))_{x_i\in S}$ is unchanged under $\cD$ compared to $\cD_S$;


\item For all $x,y\in X$, 
\begin{align*}
    \expec_{\alpha \sim \cD}[\dista(x,y)] &\leq L\cdot c_S\cdot d_X(x,y).
\end{align*}
In other words, the expected expansion under $\cD$ should be bounded by $L\cdot c_S$.
\end{enumerate}
\end{definition}


We now argue that if there are oblivious probabilistic Lipschitz extension functions of deterministic embeddings, they imply the existence of Lipschitz extensions of probabilistic embeddings.

\begin{theorem}\label{lem:oblivious-extend}
Let $f$ be an oblivious probabilistic Lipschitz extension function that maps deterministic embeddings $\alpha_S:S\xhookrightarrow{c_S} Y$ for any $Y\in \cY\cup\set{S}$ to embeddings on a set $X$ with extension factor $L$.
% embeddings $\alpha_S:S\xhookrightarrow{c_S} Y$ for any $Y\in \cY\cup\set{S}$ with extension factor $L$. 

Then consider $\cD_S:S\probembed{c_S}\cY$ and let $g$ be an algorithm that samples $\alpha_S\sim \cD_S$ and outputs $f(\alpha_S)$. Let $\cD\st$ be the distribution produced by running $g(\cD_S)$ and sampling an embedding from the resulting distribution. Then $\cD\st$ is  a Lipschitz extension of $\cD_S$ with extension factor $L$.
\end{theorem}

\begin{proof}
Note that we can sample from $\cD\st$ by sampling $\alpha_S$ from $\cD_S$ and then sampling from $f(\alpha_S)$. Further, for any $\alpha$ in the support of $f(\alpha_S)$, $(\alpha(u))_{u\in S}$ is fixed to be exactly $(\alpha_S(u))_{u\in S}$. Thus, $\cD\st$ has the same distribution on $S$ as does $\cD_S$.

Now we bound expansion for an arbitrary pair of nodes $x,y\in X\setminus S$. Define $K_u$ to be the random set equal to $\set{x\in X\setminus S:\alpha(x)=\alpha_S(u)}$ when $\alpha$ is drawn from $f(\alpha_S)$. Note that for $u\neq v\in S$, $\alpha_S(u)\neq \alpha_S(v)$ because $\alpha_S$ is expanding. This implies that the random sets $K_u$ form a random partition of $X\setminus S$.

Further, we get that the probability of any particular partition $\set{K_u}$ occurring is the same for all distributions in the image of $f$, as $f$ produces an oblivious Lipschitz extension and thus the input to $f$ cannot affect these probabilities. 

Let $u_x$ be the random variable corresponding to the $u\in S$ such that $\alpha(x)=\alpha_S(u)$. Then we get 


\begin{align*}
    \expec_{\alpha\sim \cD\st}[\dista(x,y)] &= \expec_{\set{K_u}}[\expec_{\alpha\sim \cD\st}[\dista(x,y)|\set{K_u}]] \\
    &= \expec_{\set{K_u}}[\expec_{\alpha_S\sim \cD_S}[\dista[\alpha_S](u_x,u_y)|\set{K_u}]] \\
    &\leq \expec_{\set{K_u}}[c_S\cdot d(u_x,u_y)] \\
    &\leq c_S\cdot L\cdot d(x,y).
\end{align*}

The first line comes from the law of total probability. The second line comes from the definition of $u_x$ and $u_y$. The third line comes from the fact that if $\set{K_u}$ is fixed, then $u_x$ and $u_y$ are fixed, and the fact that the expected distortion between any pair of nodes in $S$ is $c_S$ under $\alpha_S$. Note that we were able to take the expectation over $\set{K_u}$ without setting the choice of $\alpha_S\sim \cD_S$ in the first line due to the obliviousness of the Lipschitz extension. 

To see correctness of the fourth line, let $\iota$ be the identity map from $S$ to $S$. Note that $\expec_{\set{K_u}}[d(u_x,u_y)]=\expec_{\alpha\sim f(\iota)}[\dista(x,y)]$, and $f(\iota)$ is a probabilistic Lipschitz extension of the identity function with extension factor $L$. (Further, $\iota$ is in the domain of $f$ because it maps $S$ to $S\in \cY\cup\set{S}$.) \qed
\end{proof}

We note that it is essential that the probabilistic Lipschitz extension of the deterministic embedding used in the statement of the above lemma be oblivious. If this is not the case, then sampling from $\cD_S$ and then applying the extension to the resulting embedding could create a distribution with very high expansion on pairs that are not in $S$. In particular, the worst expansion between any pair of nodes in the drawn embedding can be quite high with high probability, even if the average expansion for any given pair is small. The definition of a Lipschitz extension of a deterministic embedding {\em only} requires that the final expansion in the new embedding be bounded  with respect to the {\em worst case} expansion for any pair in the original embedding. Thus, if we try to apply the arguments in Lemma \ref{lem:oblivious-extend} to a non-oblivious extension, we may not obtain the same result.


Further, we note that Algorithm 4.1 in \cite{chawla2024} in fact takes in any embedding $\alpha_S:S\xhookrightarrow{c_S}Y$ for {\em any} metric space $Y$ and samples  from an oblivious probabilistic Lipschitz extension of $\alpha_S$ with extension factor $125H_k$, where $k:=|X\setminus S|$. Thus,  Theorem \ref{lem:oblivious-extend} implies that for {\em any} $\cY$ and any $\cD_S\probembed{c_S}\cY$, there exists a Lipschitz extension $\cD$ of $\cD_S$ with extension factor $125H_k$.  



==> nest.tex <==
\section{Probabilistic nested embeddings\label{sec:nest}}


In this section we prove Theorem \ref{thm:hst-nest} by first establishing a set of properties for the existence of good probabilistic nested embeddings. We then show how to achieve these properties for HST embeddings
% developing an approach for constructing probabilistic nested embeddings into arbitrary classes of metrics. 
Recall that we are given a metric space $(X, d_X)$, a target class of metrics $\cY$, a subset $S$ with $k=|X\setminus S|$, and an assortment of probabilistic embeddings $(\cD_S, \set{\cD_{K'}}_{|K'|\leq k+1})$. Our goal is to produce a single probabilistic embedding for the entire set $X$ that has small expansion. 
% Chawla and Sheridan consider the deterministic case where we start with a deterministic embedding $\alpha_S$ from $S$ to $\cY$. At a high level, their algorithm works as follows.\footnote{We were notified after the publication of \cite{chawla2024} that the Lipschitz extension algorithm of that paper (a building block of the nested embedding algorithm presented here) is essentially the same as the rounding algorithm presented in Section 2 of Calinescu et al. \cite{calinescu2005extension}, with the following changes: (1) \cite{calinescu2005extension} use a semimetric obtained from an LP solution to the $0$-extension problem everywhere that we use $d$, (2) \cite{calinescu2005extension} pick a uniformly random permutation over $S$ (which they refer to as {\em terminals}) rather than taking a random permutation over $\gamma^{-1}(K)$ as we do here (note that $|S|=n-k$ and $|\gamma^{-1}(K)|\leq k$), and (3) \cite{calinescu2005extension} pick $b$ from the range $[1,2)$. Notably, if their algorithm is modified to use a random permutation of $\gamma^{-1}(K)$ rather than $S$, a slight modification of their analysis obtains the some of the same results that we do, with tighter constants.} It partitions the set of ``outliers'' $K=X\setminus S$ into multiple sets $K_1, K_2, \ldots$ in a certain random fashion. It also identifies for each set $K_i$ a ``close'' vertex $\gamma_i\in S$. In the composition embedding, it then maps every vertex in $K_i$ to the image of $\gamma_i$ under $\alpha_S$. 

Our approach is based on the nested embedding technique of Algorithms 4.1 and 5.1 in Chawla and Sheridan \cite{chawla2024} for $\ell_1$ embeddings but strengthens that technique by introducing a general procedure for merging embeddings. 
% Our techniques are largely based on Algorithms 4.1\footnote{We were notified after the publication of \cite{chawla2024} that the Algorithm 4.1 in that paper (a building block of the nested embedding algorithm presented here) is essentially the same as the rounding algorithm presented in Section 2 of Calinescu et al. \cite{calinescu2005extension}, with the following changes: (1) \cite{calinescu2005extension} use a semimetric obtained from an LP solution to the $0$-extension problem everywhere that we use $d$, (2) \cite{calinescu2005extension} pick a uniformly random permutation over $S$ (which they refer to as {\em terminals}) rather than taking a random permutation over $\gamma^{-1}(K)$ as we do here (note that $|S|=n-k$ and $|\gamma^{-1}(K)|\leq k$), and (3) \cite{calinescu2005extension} pick $b$ from the range $[1,2)$. Notably, if their algorithm is modified to use a random permutation of $\gamma^{-1}(K)$ rather than $S$, a slight modification of their analysis obtains the some of the same results that we do, with tighter constants.} and 5.1 from Chawla and Sheridan \cite{chawla2024}.
There are two challenges that we need to address in order to adapt these algorithms to our setting. First, we need to ensure that the final composition does not contract distances. In \cite{chawla2024}'s Algorithm 4.1, although the expansion for every pair of points can be bounded for this composition, distances can get contracted by arbitrarily large factors -- indeed some vertices end up colocated under the composition. As in \cite{chawla2024}, we randomly partition $K=X\setminus S$ into sets $K_1, K_2, \ldots$, and identify a ``close'' vertex $\gamma_i\in S$ for each such set. Then, we consider the embedding in the given assortment that maps $K_i\cup\{\gamma_i\}$ into $\cY$. We ``merge'' this embedding with the embedding $\alpha_S$ in such a fashion that neither embedding by itself gets distorted any further. This allows us to bound contraction in a similar way to Algorithm 5.1 from \cite{chawla2024}, though we frame it more generally. We then iterate in this manner over all of the components in the partition of $K$. 

The second challenge is to combine the per-pair $\alpha_S$ expansion guarantee into a expected distortion guarantee when we draw an $\alpha_S$ from the given probabilistic embedding $\cD_S$. The key property that allows us to do so is the {\em independence} of the procedure for partitioning $K$ and the structure of $\alpha_S$. We call this property {\em obliviousness} and will revisit it more formally in Appendix~\ref{sec:lip}.

We will now identify properties of the merging procedure that we require in order to obtain guarantees for the final composition.




\begin{definition}[Perfect merge]\label{def:merge-expansion}
Let $Z_1,Z_2\subseteq X$ with $Z_1\cap Z_2 = \{v\}$.
Let $\alpha_1:Z_1\rightarrow Y_1$ and $\alpha_2:Z_2\rightarrow Y_2$ be deterministic expanding embeddings, for $Y_1,Y_2\in \cY$. 
%Let $\mergeplain(\alpha,\alpha',v)$ be a function that outputs an embedding $\alpha:Z_1\cup Z_2\rightarrow Y$ for some $Y\in \cY$.
%Then we say that $\mergeplain$ is a {\em \goodmerge\ merge function} for $(X,d)$ if 
We say that a procedure $\mergeplain$  is a \goodmerge\ merge function for embedding $X$ into $\cY$ if given any pair $\alpha_1$ and $\alpha_2$ of embeddings from subsets of $X$ into $\cY$ satisfying the conditions above, it produces a an embedding $\alpha:Z_1\cup Z_2\rightarrow Y$ for some $Y\in \cY$ such that:
% We say that an embedding $\alpha:Z_1\cup Z_2 \rightarrow Y$ for some $Y\in\cY$ is a {\em \goodmerge\ merge} of $\alpha_1$ and $\alpha_2$ if
% \vspace{-.3cm}
\begin{enumerate}
    \item For all $x,y\in Z_1$, $\dista(x, y)=\dista[\alpha_1](x,y)$.
    \item For all $x,y\in Z_2$, $\dista(x, y)=\dista[\alpha_2](x,y)$.
    \item For $x\in Z_1\setminus\set{v}$ and $y\in Z_2\setminus\set{v}$, we have $\dista(x,y)\geq \max\set{\dista[\alpha_1](x,v),\dista[\alpha_2](v,y)}$.
\end{enumerate}
% We say that a procedure $\mergeplain$  is a \goodmerge\ merge function for embedding $X$ into $\cY$ if given any pair $\alpha_1$ and $\alpha_2$ of embeddings from subsets of $X$ into $\cY$ satisfying the conditions above, it produces a \goodmerge\ merge of the pair.
\end{definition}

Now we present Algorithm \ref{alg:nest} that, given an assortment of probabilistic embeddings on subsets of $X$, produces a new embedding that is drawn from a strongly nested composition of the input embeddings. We highlight in red where Algorithm \ref{alg:nest} differs from Algorithm 5.1 in \cite{chawla2024}. In \cite{chawla2024}, the input $\pmerge$ function was merely concatenation of vectors in the $\ell_1$ metric. We will develop a different \pmerge\ merge function for embeddings into HSTs in this section.



\input{algnest}



% The main result of this section is as follows.
\begin{theorem}\label{thm:merge-nested}
Let $\pmerge$ be a \goodmerge\ merge function for embeddings from $(X,d)$ into a given class $\cY$. Then, given an assortment of probabilistic embeddings $(\cD_S, \set{\cD_{K'}}_{|K'|\leq k+1})$ and the procedure $\pmerge$, Algorithm \ref{alg:nest} returns a sample from a strong probabilistic {$(3,g)$}-nested composition with $g(c_S, c_X, k) = O((c_S+ c_X(k))\cdot H_k)$, where $H_k$ is the $k$th harmonic number and $c_X(k)$ is an upper bound on the distortion for any of the $\cD_{K'}$ in the input.
\end{theorem}


We break down the proof of the theorem into two parts: bounding the expansion of the embedding (Lemma~\ref{lem:merge-expansion}) and its contraction (Lemma~\ref{lem:limit-contraction}). 

\begin{lemma}\label{lem:merge-expansion}
Let $\pmerge$ be a \goodmerge\ merge function for embeddings from $(X,d)$ into a given class $\cY$. Then, given an assortment of expanding probabilistic embeddings $(\cD_S, \set{\cD_{K'}}_{|K'|\leq k+1})$ and the procedure $\pmerge$, Algorithm \ref{alg:nest}  returns a random embedding $\alpha$ from $X$ to $\cY$ 
such that for all $x,y\in X$,
\begin{align*}
    \expec_{\alpha}[\dista(x,y)] &\leq (125\,c_S+116\, c_X(k))\cdot H_k \cdot d(x,y).
\end{align*}
Further, if $x,y\in S$, then $\expec_{\alpha}[\dista(x,y)]\leq c_S\cdot d(x,y)$.
\end{lemma}


We formally prove Lemma \ref{lem:merge-expansion}  in \ref{sec:expansionproof}. It follows essentially the same proof technique as that of Algorithm 5.1 in \cite{chawla2024}, though we pay special attention to the independence of the $\alpha_S$ we draw from $\cD_S$ and the random partitioning of $K$.

\begin{lemma}\label{lem:limit-contraction}
Let $\pmerge$ be a \goodmerge\ merge function for embeddings from $(X,d)$ into a given class $\cY$. Then, given an assortment of expanding probabilistic embeddings $(\cD_S, \set{\cD_{K'}}_{|K'|\leq k+1})$ and the procedure $\pmerge$, Algorithm \ref{alg:nest} returns an embedding $\alpha$ from $X$ to $\cY$ such that 
for all $x,y\in X$, $\dista(x,y)\geq  d(x,y)/3$.
\end{lemma}

To intuitively understand the contraction bound, note that when some node $v\in K_i$ is added to the domain of $\alpha$, there is no contraction between $v$ and other nodes in $K_i\cup \set{\gamma(u_i)}$, as $\cD_{K_i\cup\set{\gamma(u_i)}}$ is non-contracting and we use a perfect merge function to combine this with $\alpha$. Further, for any node $u$ already in the domain of $\alpha$ when $v$ was added, property 3 of perfect merge functions ensures $d_\alpha(u,v)\geq \max\set{d_\alpha(u,\gamma(u_i)),d_\alpha(v,\gamma(u_i))}$. Applying the triangle inequality and appropriate contraction bounds on $\alpha$ prior to this point gives us the result.
Notably, Lemma \ref{lem:limit-contraction} does allow a small amount of contraction, but if metrics in $\cY$ can be ``scaled up'' and stay in $\cY$ (such as when $\cY$ is the set of HSTs), we immediately get Theorem \ref{thm:merge-nested} from Lemmas \ref{lem:merge-expansion} and \ref{lem:limit-contraction}.


\begin{proofof}{Lemma~\ref{lem:limit-contraction}}
We will actually prove a slightly stronger claim about contraction: for $x,y\in X$, we have 
\begin{enumerate}
    \item If $x$ and $y$ are in $S$, then $\dista(x,y)\geq d(x,y)$.
    \item If at least one of $x,y$ is in $S$, then $\dista(x,y)\geq d(x,y)/2$.
    \item For all $x,y$, $\dista(x,y)\geq d(x,y)/3$.
\end{enumerate}
As established by Fact~\ref{lem:induct}, we need only focus on the time when $x$ and $y$ first appear in the domain of $\alpha$.
\begin{enumerate}
    \item Consider $x,y\in S$. Note $\alpha$ is first defined as $\alpha_S\from \cD_S$, so at this point $x$ and $y$ are both in its domain and $\dista(x,y)=\dista[\alpha_S](x,y)\geq d(x,y)$, by the fact that all embeddings in $\cD_S$ are expanding.
\item Now consider $x\in S,y\in X\setminus S$. We show that no matter the choice of $\set{K_j}$ (the partition of the outliers), the claim holds. In particular, consider some choice of $\set{K_j}$ with $y\in K_i$ for some $i$. Then let $\alpha_i$ be in the support of $\cD_{K_i}$, and define $\alpha'\from \pmerge(\alpha,\alpha_i)$, where $\alpha$ is the embedding at the start of this iteration in the algorithm. Also let $\gamma(u_i)$ be the vertex common to the two embeddings that are being merged. Then we get from Definition~\ref{def:merge-expansion} 
    \begin{align*}
        \dista[\alpha'](x,y) &\geq \max\set{\dista(x, \gamma(u_i)), \dista[\alpha_i](\gamma(u_i), y)} \\
        &\geq \max\set{d(x,\gamma(u_i)),d(\gamma(u_i),y)} \\
        &\geq d(x,y)/2
    \end{align*}
    where the first line is because $\pmerge$ is a \goodmerge\ merge function, the second line is by the first part of this claim and the fact that $\alpha_i$ is expanding, and the third line is by applying the triangle inequality on $d(x,y)$. 
    \item Finally, consider $x,y\in X\setminus S$. Again, fix a choice of the partition $\set{K_j}$ from the algorithm. If $x,y\in K_i$ for the same $i$, let $\alpha_i$ be in the support of $\cD_{K_i}$ and let $\alpha'\from \pmerge(\alpha,\alpha_i)$. Then $\dista[\alpha'](x,y)=\dista[\alpha_i](x,y)\geq d(x,y)$, where we used the fact that we have a \goodmerge\ merge function and $\alpha_i$ is expanding. 

    Thus, we are left with the case that $x\in K_i,y\in K_j$ for $i\neq j$. Wlog assume $i<j$. Then $x$ and $y$ first appear in the domain of $\alpha$ at iteration $j$ of the algorithm. Let $\alpha$ be the embedding before iteration $j$ and let $\alpha'$ be the embedding that results from the merge in iteration $j$. Let $\alpha_j$ be drawn from the support of $\cD_{K_j}$. Then, recalling that $x$ is in the domain of $\alpha$ prior to the merge, we get 
    \begin{align*}
        \dista[\alpha'](x,y) &\geq \max\set{\dista(x, \gamma(u_j)),\dista[\alpha_j](\gamma(u_j),y)} \\
        &\geq \max\set{d(x,\gamma(u_j))/2,d(\gamma(u_j),y)} \\
        &\geq d(x,y)/3,
    \end{align*}
    where the first line is because we have a \goodmerge\ merge function; the second line is by the second case of this claim, the fact that $\gamma(u_j)\in S$, and the fact that all embeddings in $\cD_{K_j}$ are expanding; the third is by the triangle inequality applied to $d(x,y)$. \hfill    
\end{enumerate}
\end{proofof}

% A full proof of Lemma \ref{lem:limit-contraction} is in Appendix \ref{sec:proofs}.

% The proof of the expansion lemma (Lemma~\ref{lem:merge-expansion}) follows a very similar argument to that given for Algorithm 5.1 in \cite{chawla2024}. The main difference is that it allows the input embedding $\cD_s$ to be probabilistic, and uses the fact that each $\alpha_S$ drawn from this distribution is independent of the partition $K_i$ as well as the embeddings $\alpha_i$. For completeness, we include the full proof in Appendix~\ref{sec:proofs}.
% \kristin{give outline of proof and defer the rest to the appendix}
% We will now prove Lemma~\ref{lem:limit-contraction}. An essential consequence of using a \goodmerge\ merge function with Algorithm \ref{alg:nest} is that when bounding expansion or contraction for a pair $x,y$, we need only bound this value at the point in the algorithm where they both appear in the domain of $\alpha$ for the first time. At any subsequent iteration, as $\alpha$ undergoes further merge steps, the first condition in Definition~\ref{def:merge-expansion} ensures that the distance between $x$ and $y$ stays the same. We summarize this observation in the following fact. 
% \begin{fact}\label{lem:induct}
% Let $x,y\in X$. Consider the first iteration of Algorithm~\ref{alg:nest} in which both $x$ and $y$ are in the domain of $\alpha$, and let $\hat{d}$ be $\dista(x,y)$ at that time step. Then at every subsequent iteration of the algorithm, $\dista(x,y)=\hat{d}$.
% \end{fact}
% We now proceed to bound the contraction. Note that we do get a small amount of contraction, so to actually obtain an expanding embedding, we need to be able to ``scale up'' the set of points we map to while still staying in $\cY$.
% %\begin{proofof}
% \vspace{0.1in}\noindent
% {\em Proof of Lemma~\ref{lem:limit-contraction}.~}
% We will actually prove a slightly stronger claim about contraction: for $x,y\in X$, we have 
% \begin{enumerate}
%     \item If $x$ and $y$ are in $S$, then $\dista(x,y)\geq d(x,y)$.
%     \item If at least one of $x,y$ is in $S$, then $\dista(x,y)\geq d(x,y)/2$.
%     \item For all $x,y$, $\dista(x,y)\geq d(x,y)/3$.
% \end{enumerate}
% As established by Fact~\ref{lem:induct}, we need only focus on the time when $x$ and $y$ first appear in the domain of $\alpha$.
% \begin{enumerate}
%     \item Consider $x,y\in S$. Note $\alpha$ is first defined as $\alpha_S\from \cD_S$, so at this point $x$ and $y$ are both in its domain and $\dista(x,y)=\dista[\alpha_S](x,y)\geq d(x,y)$, by the fact that all embeddings in $\cD_S$ are expanding.
% \item Now consider $x\in S,y\in X\setminus S$. We show that no matter the choice of $\set{K_j}$ (the partition of the outliers), the claim holds. In particular, consider some choice of $\set{K_j}$ with $y\in K_i$ for some $i$. Then let $\alpha_i$ be in the support of $\cD_{K_i}$, and define $\alpha'\from \pmerge(\alpha,\alpha_i)$, where $\alpha$ is the embedding at the start of this iteration in the algorithm. Also let $\gamma(u_i)$ be the vertex common to the two embeddings that are being merged. Then we get from Definition~\ref{def:merge-expansion} 
%     \begin{align*}
%         \dista[\alpha'](x,y) &\geq \max\set{\dista(x, \gamma(u_i)), \dista[\alpha_i](\gamma(u_i), y)} \\
%         &\geq \max\set{d(x,\gamma(u_i)),d(\gamma(u_i),y)} \\
%         &\geq d(x,y)/2
%     \end{align*}
%     where the first line is because $\pmerge$ is a \goodmerge\ merge function, the second line is by the first part of this claim and the fact that $\alpha_i$ is expanding, and the third line is by applying the triangle inequality on $d(x,y)$. 
%     \item Finally, consider $x,y\in X\setminus S$. Again, fix a choice of the partition $\set{K_j}$ from the algorithm. If $x,y\in K_i$ for the same $i$, let $\alpha_i$ be in the support of $\cD_{K_i}$ and let $\alpha'\from \pmerge(\alpha,\alpha_i)$. Then $\dista[\alpha'](x,y)=\dista[\alpha_i](x,y)\geq d(x,y)$, where we used the fact that we have a \goodmerge\ merge function and $\alpha_i$ is expanding. 

%     Thus, we are left with the case that $x\in K_i,y\in K_j$ for $i\neq j$. Wlog assume $i<j$. Then $x$ and $y$ first appear in the domain of $\alpha$ at iteration $j$ of the algorithm. Let $\alpha$ be the embedding before iteration $j$ and let $\alpha'$ be the embedding that results from the merge in iteration $j$. Let $\alpha_j$ be drawn from the support of $\cD_{K_j}$. Then, recalling that $x$ is in the domain of $\alpha$ prior to the merge, we get 
%     \begin{align*}
%         \dista[\alpha'](x,y) &\geq \max\set{\dista(x, \gamma(u_j)),\dista[\alpha_j](\gamma(u_j),y)} \\
%         &\geq \max\set{d(x,\gamma(u_j))/2,d(\gamma(u_j),y)} \\
%         &\geq d(x,y)/3,
%     \end{align*}
%     where the first line is because we have a \goodmerge\ merge function; the second line is by the second case of this claim, the fact that $\gamma(u_j)\in S$, and the fact that all embeddings in $\cD_{K_j}$ are expanding; the third is by the triangle inequality applied to $d(x,y)$. \hfill $\square$    
% \end{enumerate}


% Theorem~\ref{thm:merge-nested} follows almost immediately from Lemmas \ref{lem:merge-expansion} and \ref{lem:limit-contraction}, with one minor change. Technically, we defined a nested composition to be deterministically non-contracting, and here we have only shown that contraction is deterministically upper bounded by $3$. However, if the metrics in $\cY$ can be ``scaled up'' and stay in $\cY$ (such as in HSTs), we can obtain the proper definition by scaling the expansion up by an extra factor of $3$.





\subsection*{Nested embeddings for HSTs}

\input{alg_merge_hst}


We now present a \goodmerge\ merge function for HSTs.
Algorithm \ref{alg:merge} takes in two $\beta$-HSTs for a fixed ratio $\beta$ and returns another $\beta$-HST.
We show in Lemma \ref{claim:hst-merge-good} that $\merge$ is \goodmerge. 

\begin{lemma}
\label{claim:hst-merge-good}
Algorithm \ref{alg:merge} is a perfect merge function for embeddings into {$\beta$-}HSTs.
\end{lemma}




\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/merge.pdf}
    \caption{This figure depicts what happens in the algorithm $\merge$. In particular, $u$ is the node common to both HSTs on the left side of the figure. The triangles represent subtrees, and the letters below the triangles indicate the presence of the corresponding node as a leaf of that subtree. Note that after merging trees, the least common ancestor of $x$ and $y$ is that of $x$ and $u$ from the first tree, as this was higher than that of $y$ and $u$.
    % Further, the least common ancestor of $x'$ and $y'$ is at the height of the least common ancestor of $u$ and $y'$ in the second tree, as that is higher than the least common ancestor of $u$ and $x'$ in the first tree. 
    This is the foundational idea behind why  $\dista[\alpha](x,y)\geq \max\set{\dista[\alpha_1](u,x),\dista[\alpha_2](u,y)}$ holds when $\alpha$ is the output embedding for $\merge$ on inputs $\alpha_1$ and $\alpha_2$.  }
    \label{fig:merge}
\end{figure}


Figure~\ref{fig:merge} illustrates how \merge\ works. Given two HSTs that share a common leaf vertex, the function aligns the two HSTs along the path from the shared leaf to the respective roots, and merges the intermediate vertices along the way. By the manner in which we have defined $\beta$-HSTs, the lengths of the edges along the common paths align correctly with each other, enabling the guarantees we require. We defer the correctness proof for this lemma to Appendix \ref{sec:hstmergeproof}. Note that Theorem \ref{thm:merge-nested} and Lemma \ref{claim:hst-merge-good} plus the fact that all $n$-point metrics probabilistically embed into HSTs with $O(\log n)$ distortion \cite{frt04} imply Theorem \ref{thm:hst-nest}.







==> ultrametric.tex <==
\section{Ultrametrics \label{sec:ultrametric}}


We can also consider how our results affect embeddings into another popular class of metrics called ultrametrics, which are defined as follows.



\begin{definition}\label{def:ultrametrics}
A metric $(X,d)$ is an {\em ultrametric} if for all $x,y,z\in X$, $d(x,y)\leq \max\set{d(x,z),d(z,y)}$. 
\end{definition}


Note that HSTs form a subset of the set of {\em ultrametrics}. Further, because HSTs are a subset of all ultrametrics and any ultrametric embeds into an HST with distortion at most $2$ \cite{bartal2003}, we also obtain the following corollary to Theorem \ref{thm:outlier}. 

\begin{corollary}\label{cor:ultrametric-outlier}
Given a metric $(X,d)$ and target distortion $c$, let $k$ be the optimal outlier set size for probabilistically embedding $(X,d)$ into ultrametrics. Then for any constant $\epsilon>0$, there exists an algorithm that efficiently samples from a probabilistic embedding of some $S\subseteq X$ into ultrametrics with $|X\setminus S|\leq O(\frac{1}{\epsilon}k\log^2k)$ and distortion at most $(64+\epsilon)c$.
\end{corollary}


